BOND: Benchmarking Unsupervised Outlier Node Detection on Static Attributed Graphs

Detecting which nodes in graphs are outliers is a relatively new machine learning task with numerous applications. Despite the proliferation of algorithms developed in recent years for this task, there has been no standard comprehensive setting for performance evaluation. Consequently, it has been difficult to understand which methods work well and when under a broad range of settings. To bridge this gap, we present--to the best of our knowledge--the first comprehensive benchmark for unsupervised outlier node detection on static attributed graphs called BOND, with the following highlights. (1) We benchmark the outlier detection performance of 14 methods ranging from classical matrix factorization to the latest graph neural networks. (2) Using nine real datasets, our benchmark assesses how the different detection methods respond to two major types of synthetic outliers and separately to "organic" (real non-synthetic) outliers. (3) Using an existing random graph generation technique, we produce a family of synthetically generated datasets of different graph sizes that enable us to compare the running time and memory usage of the different outlier detection algorithms. Based on our experimental results, we discuss the pros and cons of existing graph outlier detection algorithms, and we highlight opportunities for future research. Importantly, our code is freely available and meant to be easily extendable: https://github.com/pygod-team/pygod/tree/main/benchmark

==> obsolete/sec05-future.tex <==
\section{Discussion and Future Directions}
\label{sec05:future}




\subsection{Future Research Directions on Graph Outlier Detection}
% \label{subsec:research_direction}
% We identify a few promising research directions for \method throughout this study. 






% on detection results.




% \subsection{Empirical Guidance for Industry Practitioners}
% (1) choose classical or deep based on the size of datasets and the number of features?
% (2) budget driven: memory and time budget?
% (4) stability driven
% (3) with knowledge on anomaly types?


% Although no-free-lunch theorem, is any algorithm perform universally well?



\vspace{-0.05in}

% \textbf{Dynamic graph}. \textcolor{blue}{remove if there is no space}

% \textbf{More types of injected outliers}. \textcolor{blue}{remove if there is no space}




==> tables/api_demo.tex <==
\begin{minipage}{0.95\linewidth}
\renewcommand{\lstlistingname}{Code demo} % Listing->Code
\begin{lstlisting}[caption={Using Dominant \citep{ding2019deep} on Cora data \citep{Morris+2020} 
% \textcolor{blue}{import the Planetoid at the top. Should we go through each lines of the code in the body text?} \textcolor{red}{I updated the caption; maybe it is fine since cora is quite popular?}
},captionpos=b, label={lst:label}, numbers=left, xleftmargin=0.5em,frame=single,framexleftmargin=1.3em]
   from pygod.utils import load_data                # import loader
   data = load_data("inj_cora")                     # load data
  
   from pygod.models import DOMINANT                # import the model
   model = DOMINANT()                               # init. detection model
   model.fit(data)                                  # fit with data
  
   pred_label = model.predict(data)                 # predict binary labels
   pred_score = model.decision_function(data)       # predict outlier scores
   pred_proba = model.predict_proba(data)           # predict probabilities
  
   from pygod.metrics import eval_roc_auc           # import eval. func.
   eval_roc_auc(y, pred_score)                      # eval. by AUC
\end{lstlisting}
\end{minipage}

==> tables/dataset-analysis.tex <==
\begin{table}[!h]
% \begin{wraptable}{l}{8.5cm}
\centering
\caption{The average neighbor similarity (\textbf{NS}) and clustering coefficient (\textbf{CC}) of outliers and inliers in different datasets. \rv{The new results in revision are highlighted in \hl{yellow}}.}
\label{tab:data-analysis}
\scalebox{0.82}{
\begin{tabular}{@{}l|cccccccccccc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Cora}} & \multicolumn{2}{c}{\textbf{Amazon}} & \multicolumn{2}{c}{\textbf{Flickr}} & \multirow{2}{*}{\textbf{Weibo}} & \multirow{2}{*}{\textbf{Reddit}} & \multirow{2}{*}{\textbf{Disney}} & \multirow{2}{*}{\textbf{Books}} & \multirow{2}{*}{\textbf{Enron}} & \multirow{2}{*}{\textbf{DGraph}}  \\
 & cont. & stru. & cont. & stru. & cont. & stru. &&&&& \\
  \midrule
\textbf{NS(inlier)} &\multicolumn{2}{c}{xxx}&\multicolumn{2}{c}{xxx}&\multicolumn{2}{c}{xxx}&0.993&0.504&OF&0.485&OF&0.162\\
\textbf{NS(outlier)} &&&&&&&0.004&0.467&OF&0.592&OF&0.071\\
\midrule
\textbf{CC(inlier)} &\multicolumn{2}{c}{xxx}&\multicolumn{2}{c}{xxx}&\multicolumn{2}{c}{xxx}&0.301&&0.214&0.241&&0.034 \\
\textbf{CC(outlier)} &&&&&&&0.400&&0.292&0.261&&0.025 \\

\bottomrule
\end{tabular}}
% \vspace{-0.1in}
\end{table}
% \end{wraptable} 
